New Convergence Aspects of Stochastic Gradient Algorithms

The classical convergence analysis of SGD is carried out under the assumption that the norm of the stochastic gradient is uniformly bounded. While this might hold for some loss functions, it is violated for cases where the objective function is strongly convex. In Bottou et al. (2018), a new analysis of convergence of SGD is performed under the assumption that stochastic gradients are bounded with respect to the true gradient norm. We show that for stochastic problems arising in machine learning such bound always holds; and we also propose an alternative convergence analysis of SGD with diminishing learning rate regime. We then move on to the asynchronous parallel setting, and prove convergence of Hogwild! algorithm in the same regime in the case of diminished learning rate. It is well-known that SGD converges if a sequence of learning rates $\{\eta_t\}$ satisfies $\sum_{t=0}^\infty \eta_t \rightarrow \infty$ and $\sum_{t=0}^\infty \eta^2_t < \infty$. We show the convergence of SGD for strongly convex objective function without using bounded gradient assumption when $\{\eta_t\}$ is a diminishing sequence and $\sum_{t=0}^\infty \eta_t \rightarrow \infty$. In other words, we extend the current state-of-the-art class of learning rates satisfying the convergence of SGD.

==> sections/Fixed_stepsize.tex <==
\subsection{Fixed stepsize}
\label{subsec:hogwild_fixedstepsize}

We consider a processor $P$ make an inconsistent read $\hat{w}_t$ of $w$  at the moment $t-\rho_t$ (i.e., $w=w_{t-\rho_t}$) and updates $w$ at the moment $t$ ($w=w_t$) with an amount of $-\eta_t \langle \nabla f(\hat{w}_t;\xi_t),e[s_t] \rangle e[s_t]$. The convergence of the sequence $\hat{w}_t$ is guaranteed if $\eta_t \leq \frac{\alpha_t\Delta}{\mu(t+E)}$ with $4 \leq \alpha_t \leq \alpha$. Assume that $t-\rho_t+E \in [2^h,2^{h+1}]$ for a certain $h$. Then, the stepsize $\eta_t$ can be fixed as $\frac{4}{\mu 2^h}$ for all $t$ such as $t-\rho_t+E \in [2^h,2^{h+1}]$. 
%and the sequence $w^t$ still converges because $\eta_t = \frac{2}{\mu 2^h} < \frac{\alpha_t}{\mu(t+E)} < \frac{\alpha}{\mu(t+E)}$. 
The reason is as follows. Since $E \geq 2R \geq 2\rho_t$ (see Assumption~\ref{Assumption:hogwild_rhot}), $\rho_t \leq t+E-\rho_t$. Therefore, $t+E=t+E-\rho_t + \rho_t \leq 2(t+E-\rho_t)$. This inequality combines with the given fact $t+E-\rho_t \leq 2^{h+1}$ yields $$t+E \leq 2^{h+2}.$$

This implies $\frac{4(t+E)}{2^h}\leq 16$. Let choose $\alpha_t \geq \frac{4(t+E)}{2^h}$ and $\alpha=16$. Since $t+E \geq t+E -\rho_t \geq 2^h$, $$\alpha_t \geq 4.$$  

Moreover, $\frac{4}{2^h} \leq \frac{\alpha_t}{t+E} \leq \frac{\alpha}{t+E}$. In other words, $\eta_t = \frac{4}{\mu 2^h} \leq \frac{\alpha_t}{\mu (t+E)} \leq \frac{\alpha}{\mu(t+E)}$. The convergence rate of the algorithm with this fixed stepsize in each period $[2^h,2^{h+1}]$ follows Theorem~\ref{theorem:Hogwild_newnew1}.

\begin{algorithm}[h!]
   \caption{Hogwild! with fixed stepsize}
   \label{algo:hogwild_fixed_stepsize}
\begin{algorithmic}
  \STATE $t \leftarrow 1$, $h \leftarrow \log_2(E)$
  \STATE Compute $\eta = \frac{4}{\mu 2^h}$
     \STATE Let Hogwild! algorithms runs
  \FOR{$t=1,2\dotsc$} 
    \STATE Increasing $t=t+1$ when a processor updates $w$ with stepsize $\eta$
    \STATE If $t+E>2^{h+1}$, then $\eta=\eta/2$ and $h=h+1$
  \ENDFOR  
\end{algorithmic}
\end{algorithm}

We describes Hogwild! with fixed stepsize in Algorithm~\ref{algo:hogwild_fixed_stepsize} for a given $E$ and $\mu$. It is worthy to highlight that SGD is a special case of the algorithm of Hogwild! described in this paper. It implies that Algorithm~\ref{algo:hogwild_fixed_stepsize} works pretty well for SGD case. Thus, we now know when and how we should diminish the stepsize to make $\hat{w}_t$ (or $w_t$) converge. 

In the previous section, we prove the convergence of Hogwild! for the diminishing stepsize $\eta_t$. In the algorithm, $\eta_t$ is required to change for every update of the shared solution $w$ and it is not so practical. Thus, Algorithm~\ref{algo:hogwild_fixed_stepsize} makes the Hogwild! with the diminishing stepsize being practical now because the user does not need to tune the stepsize for every step. It is obvious that, when $h$ is sufficient large enough, the gap between $2^h$ and $2^{h+1}$ is very large. Thus, even we have some wrong updates of variable $t$ and $h$ when the locking mechanism is not used for these variables, the convergence of $w$ is not affected. This is the most importance of Algorithm~\ref{algo:hogwild_fixed_stepsize}, i.e., the user does not to tune the stepsize or the stepsize is automatically decaying. 



 

==> sections/ack.tex <==
\section*{Acknowledgement}

The authors would like to thank the reviewers for useful suggestions which helped to improve the exposition in the paper. The authors also would like to thank Francesco Orabona for his valuable comments and suggestions. 

Lam M. Nguyen was partially supported by NSF Grants CCF 16-18717. Phuong Ha Nguyen and Marten van Dijk were supported in part by AFOSR MURI under award number FA9550-14-1-0351. Katya Scheinberg was partially supported by NSF Grants CCF 16-18717 and CCF 17-40796. Martin Tak\'{a}\v{c} was supported by  U.S. National Science Foundation, under award number NSF:CCF:1618717, NSF:CMMI:1663256 and NSF:CCF:1740796.
